Exponential asymptotics and Stokes surfaces in nonlinear three-dimensional flows

In this dissertation, we seek to expand the scope of work done by Lustri and Chapman (2013) in modelling 3D flow past a point source, in order to account for more general flows, where the strength of such a source, $\delta$, is now $O(1)$. We find that in order to solve for the Stokes surfaces of this nonlinear system, we must develop a numerical scheme to shoot from the analytically continued free surface into real space. The principal contribution of this work is a demonstration of the disparity between the line of intersection found by Lustri and Chapman (2013) and that found by our own nonlinear numerical method, along with proposed extensions for further avenues of research e.g. including surface tension.

==> abstract/abstract.tex <==
\begin{abstract}
  Abstract goes here
\end{abstract}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "thesis"
%%% End: 

==> intro/intro.tex <==
%!TEX root = ../JF-CCD.tex
\chapter{Introduction}
\label{introduction}


==> title/title.tex <==
%!TEX root = ../JF-CCD.tex

\thispagestyle{empty}
\phantomsection
\label{titlepage}
\bookmark[dest=titlepage]{Title page}
\calccentering{\unitlength}
\begin{adjustwidth*}{\unitlength}{-\unitlength}
\setlength{\parindent}{0pt}

\centering
% \flushright
\vspace*{5\onelineskip}
{
\Huge
Exponential asymptotics and\\
Stokes surfaces in nonlinear \\
three-dimensional flows \par
}
\mbox{}\rule[0pt]{0.55\textwidth}{1pt} \par  

\vspace*{1\onelineskip}
{\scshape John Fitzgerald} \\
{\itshape MMath Mathematics, University of Oxford}

\vfill 
\includegraphics[width=4cm]{blackox}
\vfill
% \begin{minipage}[t]{6cm}
% \vspace*{25pt} \flushright
% An extended essay submitted for the degree of \\
% \emph{Master of Mathematics} \\
% March 2017
% \end{minipage}\hspace*{0.2cm}
% \begin{minipage}[t]{3cm}
% \vspace*{0pt}
% \includegraphics[width=\textwidth]{blackox}
% \end{minipage}
% \begin{minipage}[t]{6cm}
% \vspace*{25pt}
A Part C Dissertation \\

Hilary Term 2018

% \end{minipage}\hspace*{0.2cm}
% \begin{minipage}[t]{3cm}
% \vspace*{0pt}
% \end{minipage}
\end{adjustwidth*}

%\newpage
%\thispagestyle{empty}
%\null
%\vfill
%\begin{quote}
%  \LARGE
%  \makebox[0pt][r]{`}\textit{Table that floats on magnets}'

%  \vfill
%  \normalsize
%  \raggedright
%  Copyright \textcopyright\ 2003--2009 Will Robertson
%  and The University of Adelaide

%  \bigskip
%  Document generated \today.

%  \bigskip
%  School of Mechanical Engineering\\
%  University of Adelaide\quad SA\\
%  Australia\quad 5005\\
%\end{quote}

%\vfill
%\begin{quotation}
%  \noindent This document has been typeset with the \LaTeX{} document
%  preparation system.

%  Page margins have been chosen as a trade-off between achieving the
%  optimal number of characters per line for ease of reading, and trying
%  to fit the typeblock onto the poorly-sized (for books), although
%  convenient, A4 stock. pdf\/\TeX's margin kerning is used to ensure optical straightness of these
%  margins.

%  If you are reading this electronically, PDF hyperlinks have
%  been automatically inserted in all appropriate positions: at
%  footnote, page number, bibliographical, figure, and table
%  references. Furthermore, bibliography entries are appended with page
%  number back references for convenience.
%\end{quotation}
%\vfill
